Query Performance Prediction using Relevance Judgments Generated by Large Language Models

Query performance prediction (QPP) aims to estimate the retrieval quality of a search system for a query without human relevance judgments. Previous QPP methods typically return a single scalar value and do not require the predicted values to approximate a specific information retrieval (IR) evaluation measure, leading to certain drawbacks: (i) a single scalar is insufficient to accurately represent different IR evaluation measures, especially when metrics do not highly correlate, and (ii) a single scalar limits the interpretability of QPP methods because solely using a scalar is insufficient to explain QPP results. To address these issues, we propose a QPP framework using automatically generated relevance judgments (QPP-GenRE), which decomposes QPP into independent subtasks of predicting the relevance of each item in a ranked list to a given query. This allows us to predict any IR evaluation measure using the generated relevance judgments as pseudo-labels. This also allows us to interpret predicted IR evaluation measures, and identify, track and rectify errors in generated relevance judgments to improve QPP quality. We predict an item's relevance by using open-source large language models (LLMs) to ensure scientific reproducibility. We face two main challenges: (i) excessive computational costs of judging an entire corpus for predicting a metric considering recall, and (ii) limited performance in prompting open-source LLMs in a zero-/few-shot manner. To solve the challenges, we devise an approximation strategy to predict an IR measure considering recall and propose to fine-tune open-source LLMs using human-labeled relevance judgments. Experiments on the TREC 2019 to 2022 deep learning tracks and CAsT-19 and 20 datasets show that QPP-GenRE achieves state-of-the-art QPP quality for both lexical and neural rankers.

==> Sections/10_Backups.tex <==
\begin{table*}[t]
\caption{
Relevance judgment agreement (Cohen's $\kappa$) between TREC assessors and each \ac{LLM}, and Pearson's $\rho$ correlation coefficients between BM25' actual nDCG@10 values and those predicted by \ourmodel integrated with each \ac{LLM} on TREC-DL 19--22.
%
The best value in each column is marked in \textbf{bold}.
%
We do not fine-tune Llama-3-70B-Instruct due to budget constraints.
}
\label{tab:finetuning}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l ll ll ll ll}
\toprule
\multirow{2}{*}{LLM}  
%& \multicolumn{8}{c}{Ranker: BM25} \\
% \cmidrule(lr){2-9}
& \multicolumn{2}{c}{TREC-DL 19} & \multicolumn{2}{c}{TREC-DL 20} & \multicolumn{2}{c}{TREC-DL 21} & \multicolumn{2}{c}{TREC-DL 22} \\
 \cmidrule(lr){2-3}  \cmidrule(lr){4-5}  \cmidrule(lr){6-7}   \cmidrule(lr){8-9}
  & \multicolumn{1}{c}{$\kappa$} & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{$\kappa$} & \multicolumn{1}{c}{P-$\rho$}   & \multicolumn{1}{c}{$\kappa$} & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{$\kappa$} & \multicolumn{1}{c}{P-$\rho$} \\
\midrule    
 GPT-3.5 (text-davinci-003)~\citep{faggioli2023perspectives} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{-}  & 0.260  & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{-} \\
  \midrule  
Llama-3.2-1B-Instruct (few-shot) & 0.013  & 0.152  & 0.029  & 0.099  & \textcolor{blue}{0.009}  & \textcolor{blue}{0.249} & \textcolor{blue}{0.079} & \textcolor{blue}{0.087} \\
\textcolor{blue}{Llama-3.2-3B-Instruct (few-shot)} & \textcolor{blue}{0.186}  & \textcolor{blue}{0.293}  &  \textcolor{blue}{0.114}  & \textcolor{blue}{0.020}  & \textcolor{blue}{0.165}  & \textcolor{blue}{0.289} & \textcolor{blue}{0.055} & \textcolor{blue}{0.443} \\
\textcolor{blue}{Mistral-7B-Instruct-v0.3 (few-shot)} & \textcolor{blue}{0.224}  & \textcolor{blue}{0.271}  & \textcolor{blue}{0.174}  & \textcolor{blue}{0.499}  & \textcolor{blue}{0.245} & \textcolor{blue}{0.414} & \textcolor{blue}{0.042} & \textcolor{blue}{0.243} \\
LLaMA-7B (few-shot) & \llap{-}0.001   & \llap{-}0.062  & \llap{-}0.003 & 0.087 &  0.003 & \llap{-}0.002 & \llap{-}0.010 & 0.214 \\
Llama-3-8B (few-shot) & 0.018   & 0.042  & 0.027 & 0.087 & 0.021 & 0.180  & \llap{-}0.035  & 0.087   \\
 Llama-3-8B-Instruct (few-shot)  & 0.315    &  0.510 & 0.227 & 0.372  & 0.238 & 0.462 & 0.049 & 0.388 \\
   \textcolor{blue}{Mistral-22B-Instruct (few-shot)} & \textcolor{blue}{0.281}   & \textcolor{blue}{0.412}   &  \textcolor{blue}{0.238}  & \textcolor{blue}{0.535}  & \textcolor{blue}{0.276} & \textcolor{blue}{0.528}  & \textcolor{blue}{0.083}  &  \textcolor{blue}{0.473} \\
   \textcolor{blue}{Llama-3-70B-Instruct (few-shot)} & \textcolor{blue}{0.321}   & \textcolor{blue}{0.526}   & \textcolor{blue}{0.245}  & \textcolor{blue}{0.557}   & \textcolor{blue}{0.279}  & \textcolor{blue}{0.545} & \textcolor{blue}{\textbf{0.086}}  & \textcolor{blue}{0.483} \\
 \midrule   
 \textcolor{blue}{Llama-3.2-1B-Instruct (fine-tuned)} & \textcolor{blue}{0.351}   & \textcolor{blue}{0.610}  &  \textcolor{blue}{0.211}  & \textcolor{blue}{0.596}  & \textcolor{blue}{0.197} & \textcolor{blue}{0.570} &  \textcolor{blue}{0.042} &  \textcolor{blue}{0.428} \\
\textcolor{blue}{Llama-3.2-3B-Instruct (fine-tuned)} & \textcolor{blue}{0.383}  & \textcolor{blue}{0.710}  & \textcolor{blue}{0.273}  & \textcolor{blue}{0.722}  & \textcolor{blue}{0.306} & \textcolor{blue}{0.608} & \textcolor{blue}{0.042} &  \textcolor{blue}{0.511}  \\
\textcolor{blue}{Mistral-7B-Instruct-v0.3 (fine-tuned)} & \textcolor{blue}{0.403}  & \textcolor{blue}{0.734}  & \textcolor{blue}{0.328}  & \textcolor{blue}{0.720}  & \textcolor{blue}{0.373} & \textcolor{blue}{0.592} & \textcolor{blue}{0.076}  & \textcolor{blue}{0.411} \\
 LLaMA-7B (fine-tuned)   &  0.258  &  \textbf{0.715}   & 0.238   & 0.627 &  0.333 & 0.547 & 0.038  & 0.388  \\
 Llama-3-8B (fine-tuned)  &  0.381  &  0.544 & \textbf{0.342}  & 0.681 & 0.347 & 0.612  & 0.082 & 0.568 \\
 Llama-3-8B-Instruct (fine-tuned) & 0.397   & 0.647   & 0.316 & \textbf{0.743}  & \textbf{0.418}  & \textbf{0.699} & 0.066  & \textbf{0.573}   \\ 
  \textcolor{blue}{Mistral-22B-Instruct (fine-tuned)} & \textcolor{blue}{\textbf{0.407}}  & \textcolor{blue}{0.682}  & \textcolor{blue}{0.276}  &  \textcolor{blue}{0.640}  & \textcolor{blue}{0.310} & \textcolor{blue}{0.591} & \textcolor{blue}{0.071} & \textcolor{blue}{0.462}  \\
  \bottomrule
\end{tabular}
\end{table*}

\if0
\begin{table*}[t]
\caption{
Relevance judgment agreement (Cohen's $\kappa$) between TREC assessors and each \ac{LLM}, and Pearson's $\rho$ correlation coefficients between BM25' actual nDCG@10 values and those predicted by \ourmodel integrated with each \ac{LLM} on TREC-DL 19--22.
%
The best value in each column is marked in \textbf{bold}.
}
\label{tab:finetuning}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l cccc}
\toprule
\multirow{2}{*}{LLM} 
%& \multicolumn{8}{c}{Ranker: BM25} \
% \cmidrule(lr){2-9}
& \multicolumn{1}{c}{TREC-DL 19} 
& \multicolumn{1}{c}{TREC-DL 20} 
& \multicolumn{1}{c}{TREC-DL 21} 
& \multicolumn{1}{c}{TREC-DL 22} \\
& \multicolumn{1}{c}{$\kappa$} 
& \multicolumn{1}{c}{$\kappa$} 
& \multicolumn{1}{c}{$\kappa$} 
& \multicolumn{1}{c}{$\kappa$} \\
\midrule
 GPT-3.5 (text-davinci-003)~\citep{faggioli2023perspectives} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}   & 0.260   & \multicolumn{1}{c}{-} \\
  \midrule  
   LLaMA-7B (few-shot) & \llap{-}0.001     & \llap{-}0.003  &  0.003  & \llap{-}0.010  \\
 % Mistral-7B (few-shot) &   &   &   &   &  &  &  &  \\
 Llama-3-8B (few-shot) & 0.018   & 0.027  & 0.021   & \llap{-}0.035    \\
 Llama-3-8B-Instruct (few-shot)  & 0.315    & 0.227   & 0.238  & 0.049 \\

 \midrule   
 LLaMA-7B (fine-tuned)   &  0.258    & 0.238    &  0.333  & 0.038    \\
% Mistral-7B (fine-tuned) &   &   &   &   &  &  &  &  \\
 Llama-3-8B (fine-tuned)  &  0.381   & \textbf{0.342}   & 0.347   & \textbf{0.082}  \\
 Llama-3-8B-Instruct (fine-tuned) & \textbf{0.397}      & 0.316  & \textbf{0.418}   & 0.066    \\ 
\bottomrule
\end{tabular}
\end{table*}
\fi


\if0
\subsection{Data leakage}
It is important to ensure LLaMA~\citep{touvron2023llama2,touvron2023llama} is not exposed to the relevance labels of the TREC-DL sets during pre-training.
\citet{touvron2023llama} clearly show the various sources used for pretraining LLaMA, such as English CommonCrawl, Wikipedia and Stack Exchange. 
There is no specific overlap with our evaluation set.
Moreover, Table~\ref{tab:finetuning} shows the poor performance of non-fine-tuned LLaMA in judging relevance, further implying that LLaMA may not have been exposed to the human relevance labels in our evaluation sets during pre-training.
%, we refer to the performance of LLaMA in the few-shot setting; see . 
%The poor performance of LLaMA in relevance judgment generation without fine-tuning, in a few-shot learning setting, confirms this statement.
\fi


\begin{table}[!t]
\centering
\caption{Relevance judgment agreement (Cohen's $\kappa$) between TREC assessors and each method, and Pearson's $\rho$ correlation coefficients between RR@10 values of BM25 and performance predicted by each method on TREC-DL 19--22.
}
\label{tab:finetuning}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{ll c c c} 
\toprule
\multirow{1}{*}{Dataset} & \multirow{1}{*}{Method} & \multirow{1}{*}{Cohen’s $\kappa$}  & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{K-$\tau$}    \\
\midrule
\multirow{2}{*}{TREC-DL 19} & LLaMA-7B (few-shot) & 0.121   & 0.281  \\
& LLaMA-7B (few-shot)  & & & \\
& Llama-3-8B (few-shot) & & & \\
& Llama-3-8B-Instruct (few-shot) & & & \\
& LLaMA-7B (fine-tuned)  & 0.258  & 0.538 & 0.486  \\
& Llama-3-8B (fine-tuned)  & & & \\
& Llama-3-8B-Instruct (fine-tuned)  & 0.397 & 0.591 & 0.535 \\ 
& RankLLaMA  &   &   &  \\
\midrule
\multirow{2}{*}{TREC-DL 20} & LLaMA-7B (few-shot) & 0.110  & 0.255  &  \\
& LLaMA-7B (fine-tuned)  & 0.238  & 0.560  & \\
\midrule
\multirow{3}{*}{TREC-DL 21} & GPT-3.5 (text-davinci-003)~\citep{faggioli2023perspectives} &  0.260  & &  - \\
& LLaMA-7B (few-shot) & 0.140  & 0.237 & \\
& LLaMA-7B (fine-tuned)  & 0.333  & 0.524  &  \\
& Llama-3-8B-Instruct (fine-tuned)  & 0.316 & 0.591 & 0.535 \\
\midrule
\multirow{2}{*}{TREC-DL 22}& LLaMA-7B (few-shot) & 0.009  & 0.109   & \\
& LLaMA-7B (fine-tuned)  & 0.190  & 0.350  & \\
\bottomrule
\end{tabular}
%}
\end{table}



\begin{table}[h]
\caption{
Correlation coefficients (Pearson's $\rho$, Kendall's $\tau$, and Spearman's $\rho$) between actual retrieval quality, in terms of MRR@10, of TCT-ColBERTv2 and performance predicted by \ourmodel/baselines, on TREC-DL 19, 20.
All coefficients are statistically significant (t-test, $p < 0.05$) except the ones in \emph{italics}.
The best value in each column is marked in \textbf{bold}.
}   
\label{tab:RQ1}
\begin{tabular}{l rrr rrr}
\toprule  
\multirow{2}{*}{QPP method}  & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20}  \\  
 \cmidrule(lr){2-4}  \cmidrule(lr){5-7} 
  & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$}  \\    
\midrule   
 Clarity & \textit{-0.140} & \textit{-0.095} & \textit{-0.118} & \textit{-0.057} & \textit{-0.027} & \textit{-0.036}\\ 
 WIG    & \textit{0.014}  & \textit{-0.034} & \textit{-0.040} & \textit{0.023}  & \textit{-0.004} & \textit{-0.011} \\
 NQC & \textit{0.211} & \textit{0.144}  & \textit{0.170}  & \textit{0.210} & \textit{0.158}  & \textit{0.210} \\     
 $\sigma_{max}$ & \textit{0.028}  & \textit{0.006} & \textit{0.011} & \textit{0.067} & \textit{0.056}  & \textit{0.074} \\    
 n($\sigma_{x\%}$) & \textit{-0.070} & \textit{-0.103} & \textit{-0.128} & \textit{-0.147} & \textit{-0.174} & \textit{-0.226} \\
 SMV & \textit{0.130} & \textit{0.083} & \textit{0.098} & \textit{0.198} & \textit{0.147} & \textit{0.193} \\ 
\ac{QPP-PRP} &  &  &  &  &  &    \\
\midrule 
 NQA-QPP & \textit{0.001} & \textit{0.010} & \textit{0.019} & \textit{0.090} & \textit{0.089}  & \textit{0.112}    \\ 
 %NQA-QPP (train) & \textit{0.210} & \textit{0.127} & \textit{0.149} & \textit{0.184} & \textit{0.109} &  \textit{0.144}   \\
BERTQPP  & \textit{0.218}  & \textit{0.184}  & \textit{0.232} & \textit{0.114}  & \textit{0.096}  & \textit{0.122}   \\
% BERTQPP (train) & -0.173  & -0.156 & -0.195 &  0.058 & 0.060 & 0.078    \\
 qppBERT-PL & \textit{-0.005} & \textit{-0.049} & \textit{-0.050} & \textit{-0.013}  & \textit{-0.008} & \textit{-0.008} \\
 \ac{M-QPPF} &  &  &  &  &  &   \\
 \midrule
\ourmodel & \textit{0.253}  & \textit{0.240}  & \textit{0.258}  & \textit{0.079}  & \textit{0.047} & \textit{0.054}   \\
  \bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\caption{
Correlation coefficients (Pearson's $\rho$, Kendall's $\tau$, and Spearman's $\rho$) between actual retrieval quality, in terms of nDCG@10, of TCT-ColBERTv2 and performance predicted by \ourmodel/baselines, on TREC-DL 19, 20.
All coefficients are statistically significant (t-test, $p < 0.05$) except the ones in \emph{italics}.
The best value in each column is marked in \textbf{bold}.
}   
\label{tab:RQ1}
\begin{tabular}{l rrr rrr}
\toprule  
\multirow{2}{*}{QPP method}  & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20}  \\  
 \cmidrule(lr){2-4}  \cmidrule(lr){5-7} 
  & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$}  \\    
\midrule  
 Clarity  & \textit{0.168} & \textit{0.102} & \textit{0.168} & \textit{0.117}  & \textit{0.096}  & \textit{0.138} \\ 
 WIG     & 0.351 & 0.259 & 0.365 & 0.375  & 0.298 & 0.419 \\ 
 NQC  & 0.392  & 0.266 & 0.377 & 0.481  & 0.352 & 0.497 \\    
 $\sigma_{max}$  & 0.318 & \textit{0.202}  & 0.303 & 0.415 & 0.321  & 0.448\\    
 n($\sigma_{x\%}$)  & \textit{0.185} & \textit{0.089} & \textit{0.151} & \textit{0.201}  & \textit{0.126} & \textit{0.183} \\
 SMV  & 0.380 & 0.264 & 0.370 & 0.464 & 0.332  & 0.459 \\ 
\ac{QPP-PRP} &  &  &  &  &  &    \\
\midrule    
 NQA-QPP & \textit{0.032} & \textit{0.066} & \textit{0.083} & \textit{0.207}  & \textit{0.147}  &  \textit{0.224}   \\
 BERTQPP & \textit{0.226} & \textit{0.120} & \textit{0.189} &  0.302 & 0.217  &  0.315  \\
 qppBERT-PL & \textit{0.125} & \textit{0.067} & \textit{0.086} & \textit{0.073} & \textit{0.082} & \textit{0.099} \\
 \ac{M-QPPF} &  &  &  &  &  &   \\
 \midrule
\ourmodel & 0.416  & 0.285  & 0.386  & 0.438 & 0.318 & 0.451   \\
  \bottomrule
\end{tabular}
\end{table} 

\begin{table}[t]
\caption{
Correlation coefficients (Pearson's $\rho$, Kendall's $\tau$, and Spearman's $\rho$) between actual retrieval quality, in terms of Recall@100, of ANCE and performance predicted by \ourmodel/baselines, on TREC-DL 19, 20.
All coefficients are statistically significant (t-test, $p < 0.05$) except the ones in \emph{italics}.
The best value in each column is marked in \textbf{bold}.
}   
\label{tab:RQ1}
\begin{tabular}{l rrr rrr}
\toprule
\multirow{2}{*}{QPP method}  & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20}  \\  
 \cmidrule(lr){2-4}  \cmidrule(lr){5-7} 
  & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$}  \\    
\midrule 
 Clarity & \textit{0.108}  & \textit{0.074} & \textit{0.110} & \textit{0.034} & \textit{0.001} & \textit{-0.004} \\ 
 WIG    & 0.416 & 0.275 & 0.399 & 0.324 & 0.258 & 0.392  \\
 NQC & 0.573 & 0.393  & 0.531 & 0.588 & 0.443 & 0.610   \\   
 $\sigma_{max}$ & 0.450 & 0.328 & 0.450 & 0.596 & 0.487  & 0.653 \\   
 n($\sigma_{x\%}$) & \textit{0.162} & \textit{0.156}  & \textit{0.231} & \textit{0.200} & \textit{0.141} & \textit{0.210}   \\
 SMV & 0.523 & 0.342 & 0.490  & 0.506 & 0.386 &  0.533 \\ 
\ac{QPP-PRP} &  &  &  &  &   &    \\
\midrule  
 NQA-QPP &  \textit{0.057} & \textit{0.159} & \textit{0.204} & 0.324  & 0.277  & 0.412     \\
 %NQA-QPP (train) & 0.301 & 0.230 & 0.320 & 0.335 &  0.342 &  0.462   \\
 BERTQPP & \textit{0.303} & \textit{0.123} & \textit{0.164} & 0.357 & 0.263  &  0.385  \\
%BERTQPP (train) & nan  & nan & nan & nan  & nan  & nan  \\
 qppBERT-PL & \textit{0.192} & \textit{0.150} & \textit{0.181} & \textit{0.192}  & \textit{0.176} & \textit{0.211} \\
 \ac{M-QPPF} &  &  &  &  &  &   \\
 \midrule
\ourmodel & \textit{0.268}   & \textit{0.184}   & \textit{0.241}   & 0.342 & 0.285 &  0.364  \\
  \bottomrule
\end{tabular}
\end{table}


\begin{table}[t]
\caption{
Correlation coefficients (Pearson's $\rho$, Kendall's $\tau$, and Spearman's $\rho$) between actual retrieval quality, in terms of Recall@100, of TCT-ColBERTv2 and performance predicted by \ourmodel/baselines, on TREC-DL 19, 20.
All coefficients are statistically significant (t-test, $p < 0.05$) except the ones in \emph{italics}.
The best value in each column is marked in \textbf{bold}.
}   
\label{tab:RQ1}   
\begin{tabular}{l rrr rrr}
\toprule    
\multirow{2}{*}{QPP method}  & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20}  \\   
 \cmidrule(lr){2-4}  \cmidrule(lr){5-7} 
  & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$}  \\    
\midrule 
 Clarity  & \textit{0.110} & \textit{0.091}  &  \textit{0.161} & \textit{0.150} & \textit{0.130} & \textit{0.172} \\ 
 WIG     & 0.378  & 0.288  & 0.397  & 0.495  & 0.351  & 0.490 \\ 
 NQC  & 0.536  & 0.375  & 0.512 & 0.605 & 0.499  & 0.656 \\    
 $\sigma_{max}$ & 0.415 & 0.270  & 0.392 & 0.640 & 0.531 & 0.695 \\    
 n($\sigma_{x\%}$)  & \textit{0.152}  & \textit{0.107} & \textit{0.143}  & 0.296 & \textit{0.182}  & \textit{0.246} \\
 SMV & 0.482  & 0.308 & 0.443 & 0.545 & 0.424  & 0.565 \\ 
\ac{QPP-PRP} &  &  &  &  &  &    \\
\midrule 
 NQA-QPP & \textit{-0.167} & \textit{-0.009} & \textit{-0.007} & 0.289  & 0.290  &  0.392   \\
 BERTQPP & \textit{0.023} & \textit{0.071} & \textit{0.093} & 0.361  & 0.216  & 0.306   \\
 qppBERT-PL & 0.319 & 0.273 & 0.342  & 0.377 & 0.288  & 0.350 \\
 \ac{M-QPPF} &  &  &  &  &  &   \\
 \midrule
\ourmodel & \textit{0.028}  & \textit{0.012}  & \textit{0.017}  & 0.342 & 0.198 & 0.277   \\
  \bottomrule
\end{tabular}
\end{table}












rr@10
dl19 bm25
llama-7b-few
llama-7b-fine  0.258    0.538 0.486

llama-13b-few
llama-13b-fine         0.446  0.388
checkpoint-930.k1000-n200-mrr@10.mrr@10: {'Pearson': 0.208, 'Kendall': 0.14
checkpoint-1860.k1000-n10-mrr@10.mrr@10: {'Pearson': 0.42, 'Kendall': 0.318,
checkpoint-2790.k1000-n1000-mrr@10.mrr@10: {'Pearson': 0.38, 'Kendall': 0.327,
checkpoint-3720.k1000-n10-mrr@10.mrr@10: {'Pearson': 0.446, 'Kendall': 0.388
checkpoint-4650.k1000-n200-map@100.mrr@10: {'Pearson': 0.306, 'Kendall': 0.209

llama-33b-few
llama-33b-fine   

llama-65b-few  
llama-65b-fine 

dl20 bm25

llama-7b-few
llama-7b-fine  0.560 0.475

llama-13b-few
llama-13b-fine  0.515 0.454
checkpoint-930.k1000-n100-mrr@10.mrr@10: {'Pearson': 0.456, 'Kendall': 0.371, 
checkpoint-1860.k1000-n100-mrr@10.mrr@10: {'Pearson': 0.396, 'Kendall': 0.334
checkpoint-2790.k1000-n400-mrr@10.mrr@10: {'Pearson': 0.515, 'Kendall': 0.454, 'Spearman': 0.538,
checkpoint-3720.k1000-n25-mrr@10.mrr@10: {'Pearson': 0.435, 'Kendall': 0.363


llama-33b-few
llama-33b-fine   

llama-65b-few
llama-65b-fine 


dl19 ance 
llama-7b-few
llama-7b-fine  0.567 0.440

llama-13b-few  
llama-13b-fine  0.509  0.409
checkpoint-930.k1000-n400-mrr@10.mrr@10: {'Pearson': 0.369, 'Kendall': 0.309,
checkpoint-1860.k1000-n100-mrr@10.mrr@10: {'Pearson': 0.366, 'Kendall': 0.269
checkpoint-2790.k1000-n100-mrr@10.mrr@10: {'Pearson': 0.446, 'Kendall': 0.386
checkpoint-3720.k1000-n200-mrr@10.mrr@10: {'Pearson': 0.509, 'Kendall': 0.409
checkpoint-4650.k1000-n400-mrr@10.mrr@10: {'Pearson': 0.342, 'Kendall': 0.265, 

 
llama-33b-few
llama-33b-fine   

llama-65b-few
llama-65b-fine 

dl20 ance

llama-7b-few
llama-7b-fine  0.293 0.257

llama-13b-few
llama-13b-fine   0.286   0.245
checkpoint-930.k1000-n1000-mrr@10.mrr@10: {'Pearson': 0.194, 'Kendall': 0.139,
checkpoint-1860.k1000-n500-mrr@10.mrr@10: {'Pearson': 0.289, 'Kendall': 0.236
checkpoint-2790.k1000-n50-mrr@10.mrr@10: {'Pearson': 0.212, 'Kendall': 0.194, 'Spearman': 0.216,
checkpoint-3720.k1000-n100-mrr@10.mrr@10: {'Pearson': 0.286, 'Kendall': 0.245,

llama-33b-few
llama-33b-fine   
 
llama-65b-few
llama-65b-fine 














\begin{table}[!t]
\centering
\caption{Actual retrieval quality of retrievers used in this paper regarding MRR@10.}
\label{table:actual}
%\setlength{\tabcolsep}{0.8mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l@{}c c c c} 
\toprule
\multirow{1}{*}{} & \multicolumn{1}{c}{TREC-DL 2019}  & \multicolumn{1}{c}{TREC-DL 2020}  & \multicolumn{1}{c}{TREC-DL 2021} & \multicolumn{1}{c}{TREC-DL 2022}   \\ 
%\cmidrule(lr){2-2} \cmidrule(lr){3-3}  \cmidrule(lr){4-4}
% & nDCG@3  & nDCG@3  & nDCG@3 \\ 
\midrule
BM25  & 0.702   & 0.653  & 0.498 & 0.312\\
ANCE   & 0.834       & 0.787       &      &     \\
%TCT-ColBERTv2 & 0.886    & 0.839     &   & \\
%BM25+MonoT5  & 0.877    & 0.839    & 0.813   & 0.673\\

\bottomrule
\end{tabular}
}
\end{table}


\begin{table}[!t]
\centering
\caption{Data statistics.}
\label{table:data}
%\setlength{\tabcolsep}{0.8mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l@{}rrrr}
\toprule
& TREC-DL 19  & TREC-DL 20 & TREC-DL 21  & TREC-DL 22\\ 
\midrule
%\#questions  & 200  & 200  & 477 &  500   \\
\#human-judged question & 43  & 54 & 53 & 76  \\
%\#passages & \multicolumn{2}{c}{8.8M}  &\multicolumn{2}{c}{138.4M}   \\
\bottomrule
\end{tabular}
}
\end{table}


To test for the statistical significance of the results, we follow \citet{faggioli2023towards} to apply one-way \ac{ANOVA}~\citep{rutherford2011anova} with \ac{HSD} post-hoc comparison procedure~\citep{tukey1949comparing}.


\begin{table*}[!t]
\centering
\caption{\ac{QPP} effectiveness of different relevance judgment generators, and relevance judgment agreement between TREC assessors and each relevance judgment generator on TREC-DL 19.
}
\label{table:actual}
%\setlength{\tabcolsep}{0.8mm}
%\resizebox{\linewidth}{!}{%
\begin{tabular}{l c cccc cccc} 
\toprule
\multirow{3}{*}{Relevance judgment generators} & \multirow{3}{*}{Cohen’s $\kappa$}  & \multicolumn{4}{c}{Target metric: RR@10} & \multicolumn{4}{c}{Target metric: nDCG@10} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} 
& \multicolumn{1}{c}{} & \multicolumn{2}{c}{Rranker: BM25} & \multicolumn{2}{c}{Rranker: ANCE}  & \multicolumn{2}{c}{Rranker: BM25} & \multicolumn{2}{c}{Rranker: ANCE} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
 &\multicolumn{1}{c}{}  & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{K-$\tau$}   & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{K-$\tau$}  & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{K-$\tau$}  \\ 
%\cmidrule(lr){2-2} \cmidrule(lr){3-3}  \cmidrule(lr){4-4}
\midrule
%\ourmodel (LLaMA-7B-zero-shot)  & 0.001  &  & &  & &  & &  & \\
\ourmodel (LLaMA-7B-few-shot) &   &  & &  & &  & &  &\\
\ourmodel (LLaMA-7B-finetuning)  & 0.258  &  & &  & &  & &  & \\
%\ourmodel (LLaMA-13B)  &   &  &     &     \\
%\ourmodel (LLaMA-33B)  &   &    &      &     \\
%\ourmodel (LLaMA-65B)  &   &   &      &     \\
\bottomrule
\end{tabular}
%}
\end{table*}

\begin{table*}[!t]
\centering
\caption{\ac{QPP} effectiveness of different relevance judgment generators, and relevance judgment agreement between TREC assessors and each relevance judgment generator on TREC-DL 20.
}
\label{table:actual}
%\setlength{\tabcolsep}{0.8mm}
%\resizebox{\linewidth}{!}{%
\begin{tabular}{l c cccc cccc} 
\toprule
\multirow{3}{*}{Relevance judgment generators} & \multirow{3}{*}{Cohen’s $\kappa$}  & \multicolumn{4}{c}{Target metric: RR@10} & \multicolumn{4}{c}{Target metric: nDCG@10} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} 
& \multicolumn{1}{c}{} & \multicolumn{2}{c}{Rranker: BM25} & \multicolumn{2}{c}{Rranker: ANCE}  & \multicolumn{2}{c}{Rranker: BM25} & \multicolumn{2}{c}{Rranker: ANCE} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
 &\multicolumn{1}{c}{}  & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{K-$\tau$}   & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{K-$\tau$}  & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{K-$\tau$}  \\ 
%\cmidrule(lr){2-2} \cmidrule(lr){3-3}  \cmidrule(lr){4-4}
\midrule
%\ourmodel (LLaMA-7B-zero-shot)  & 0.001  &  & &  & &  & &  & \\
\ourmodel (LLaMA-7B-few-shot) &   &  & &  & &  & &  &\\
\ourmodel (LLaMA-7B-finetuning)  & 0.238  &  & &  & &  & &  & \\
%\ourmodel (LLaMA-13B)  &   &  &     &     \\
%\ourmodel (LLaMA-33B)  &   &    &      &     \\
%\ourmodel (LLaMA-65B)  &   &   &      &     \\
\bottomrule
\end{tabular}
%}
\end{table*}

\begin{table*}[!t]
\centering
\caption{\ac{QPP} effectiveness of different relevance judgment generators, and relevance judgment agreement between TREC assessors and each relevance judgment generator on TREC-DL 21.
}
\label{table:actual}
%\setlength{\tabcolsep}{0.8mm}
%\resizebox{\linewidth}{!}{%
\begin{tabular}{l c cccc} 
\toprule
\multirow{2}{*}{Relevance judgment generators} & \multirow{2}{*}{Cohen’s $\kappa$}  & \multicolumn{2}{c}{Target metric: RR@10} & \multicolumn{2}{c}{Target metric: nDCG@10} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} 
 &\multicolumn{1}{c}{}  & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{K-$\tau$}   & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$}   \\ 
%\cmidrule(lr){2-2} \cmidrule(lr){3-3}  \cmidrule(lr){4-4}
\midrule
GPT-3.5 (text-davinci-003)~\citep{faggioli2023perspectives} &  0.260  & - & -& - &-\\
%\ourmodel (LLaMA-7B-zero-shot)  & 0.002  &  & &  & \\
\ourmodel (LLaMA-7B-few-shot) &   &  & &  & \\
\ourmodel (LLaMA-7B-finetuning)  & 0.333  &  & &  & \\
%\ourmodel (LLaMA-13B)  &   &  &     &     \\
%\ourmodel (LLaMA-33B)  &   &    &      &     \\
%\ourmodel (LLaMA-65B)  &   &   &      &     \\
\bottomrule
\end{tabular}
%}
\end{table*}

\begin{table*}[!t]
\centering
\caption{\ac{QPP} effectiveness of different relevance judgment generators, and relevance judgment agreement between TREC assessors and each relevance judgment generator on TREC-DL 22.
}
\label{table:actual}
%\setlength{\tabcolsep}{0.8mm}
%\resizebox{\linewidth}{!}{%
\begin{tabular}{l c cccc} 
\toprule
\multirow{2}{*}{Relevance judgment generators} & \multirow{2}{*}{Cohen’s $\kappa$}  & \multicolumn{2}{c}{Target metric: RR@10} & \multicolumn{2}{c}{Target metric: nDCG@10} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
 &\multicolumn{1}{c}{}  & \multicolumn{1}{c}{P-$\rho$}  & \multicolumn{1}{c}{K-$\tau$}   & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$}  \\ 
%\cmidrule(lr){2-2} \cmidrule(lr){3-3}  \cmidrule(lr){4-4}
\midrule
%\ourmodel (LLaMA-7B-zero-shot)  &   &  & &  & \\
\ourmodel (LLaMA-7B-few-shot) &   &  & &  & \\
\ourmodel (LLaMA-7B-finetuning)  &   &  & &  &  \\
%\ourmodel (LLaMA-13B)  &   &  &     &     \\
%\ourmodel (LLaMA-33B)  &   &    &      &     \\
%\ourmodel (LLaMA-65B)  &   &   &      &     \\
\bottomrule
\end{tabular}
%}
\end{table*}




\begin{table*}[t]
\centering
\caption{
Overview of TREC-DL 2021 relevance judgment agreement between human assessors and each of the \acp{LLM}.
}
\label{main_table} 
\begin{tabular}{ll llc}
\toprule
\multirow{2}{*}{\textbf{LLMs}} & \multirow{2}{*}{\textbf{Levels}} & \multicolumn{2}{c}{Human Assessors} & \multirow{2}{*}{Cohen’s $\kappa$} \\
\cmidrule(lr){3-4} 
  & \multicolumn{1}{c}{} & Rel. & Irrel. & \multicolumn{1}{c}{} \\
\midrule
\multirow{2}{*}{}   
& Rel. &   &   &    \multirow{2}{*}{xx} \\ 
& Irrel. &   &    \\
\midrule
\multirow{2}{*}{}   
& Rel. &   &      & \multirow{2}{*}{xx} \\ 
& Irrel. &   &     \\

\midrule

\bottomrule
\end{tabular}
%}
\vspace*{2mm}
\end{table*}


\begin{table*}[]
\caption{
Correlation coefficients (Pearson's $\rho$, Kendall's $\tau$, and Spearman's $\rho$) between actual retrieval quality, in terms of MRR@10, of BM25 and performance predicted by \ourmodel/baselines, on TREC-DL 19, 20, 21 and 22.
All coefficients are statistically significant (t-test, $p < 0.05$) except the ones in \emph{italics}.
The best value in each column is marked in \textbf{bold}.
}
\label{tab:RQ1}
\begin{tabular}{l rrr rrr rrr rrr}
\toprule
\multirow{2}{*}{QPP method}  & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20} & \multicolumn{3}{c}{TREC-DL 21} & \multicolumn{3}{c}{TREC-DL 22} \\
 \cmidrule(lr){2-4}  \cmidrule(lr){5-7}  \cmidrule(lr){8-10}   \cmidrule(lr){11-13}
  & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} \\
\midrule    
 Clarity & \textit{0.135} & \textit{0.028} & \textit{0.053} & \textit{0.050} & \textit{0.021}  & \textit{0.028} & \textit{0.183} & \textit{0.161}  & \textit{0.220}  & 0.253 &  \textit{0.099}  &\textit{0.147} \\ 
 WIG & \textit{0.113} & \textit{0.164}  & \textit{0.207} & 0.286 & 0.218 & 0.281 & \textit{0.237} & 0.206  & 0.272  & \textit{0.029} & \textit{0.082} & \textit{0.099} \\  
 NQC & \textit{0.194} & \textit{0.117} & \textit{0.153} & \textit{0.152}  & \textit{0.191}  & \textit{0.244}  & \textit{0.227} & \textit{0.195} & \textit{0.258}   & \textit{0.223} & \textit{0.048} & \textit{0.070} \\
 $\sigma_{max}$ & \textit{0.195} & \textit{0.164} & \textit{0.215} & \textit{0.200}  & 0.211  & 0.279  & 0.278  & \textit{0.174}  & \textit{0.237}  & \textit{0.038}  & \textit{0.048}  & \textit{0.064} \\  
 n($\sigma_{x\%}$)  & \textit{0.144}  & \textit{0.181} & \textit{0.226}  & \textit{0.187}  & \textit{0.123}  & \textit{0.162}  & \textit{0.127} & \textit{0.140}  & \textit{0.193}  & \textit{0.169} & \textit{0.113} & \textit{0.142} \\
 SMV  & \textit{0.141}  & \textit{0.097}  & \textit{0.132} & \textit{0.126} & \textit{0.193}  & \textit{0.245} & \textit{0.240} & \textit{0.189} & \textit{0.253}   &0.227 & \textit{0.094} & \textit{0.126}\\ 
\ac{QPP-PRP} &  &  &  &  &  &  &  &  &   &  &  &   \\
\midrule       
 NQA-QPP & \textit{0.181} & \textit{0.122} & \textit{0.149} & \textit{0.062} & \textit{0.069} & \textit{0.089} & \textit{0.161} & \textit{0.163} & \textit{0.213}  & \textit{0.224} & 0.177 & 0.239   \\   
 %NQA-QPP (train) & \textit{0.166}  & \textit{0.100}  & \textit{0.125} &  \textit{0.068} & \textit{0.133} & \textit{0.183} &  &  &   &  &  &    \\ 
 BERTQPP & \textit{0.281} & \textit{0.136}  & \textit{0.173}  & \textit{0.237}  & \textit{0.155} & \textit{0.206} &  \textit{0.206}  & \textit{0.134}  & \textit{0.187}  & \textit{0.148}  & \textit{0.122} & \textit{0.166}   \\  
 %BERTQPP (train) & 0.316 & \textit{0.228} & \textit{0.295} & 0.362 & 0.313  & 0.411 &  0.294 & \textit{0.140} & \textit{0.200}  & 0.376 & 0.204  & 0.270    \\
  qppBERT-PL & \textit{0.145}  & \textit{0.138} & \textit{0.149} & \textit{0.166} & \textit{0.152} & \textit{0.166} & 0.339 & 0.244  & 0.320  & \textit{0.131}  & 0.206 & 0.252 \\
 \ac{M-QPPF} &  &  &  &  &  &  &  &  &   &  &  &  \\
 \midrule  
\ourmodel & \textbf{0.538} & \textbf{0.486} & \textbf{0.520} & \textbf{0.560} & \textbf{0.475}  & \textbf{0.568} & \textbf{0.469} & \textbf{0.385} & \textbf{0.423}  &\textbf{0.350} & \textbf{0.262}  & \textbf{0.317} \\
  \bottomrule
\end{tabular}
\end{table*}


\begin{table}[]
\caption{
Correlation coefficients (Pearson's $\rho$, Kendall's $\tau$, and Spearman's $\rho$) between actual retrieval quality, in terms of MRR@10, of ANCE and performance predicted by \ourmodel/baselines, on TREC-DL 19, 20.
All coefficients are statistically significant (t-test, $p < 0.05$) except the ones in \emph{italics}.
The best value in each column is marked in \textbf{bold}.
}   
\label{tab:RQ1}
\begin{tabular}{l rrr rrr}
\toprule
\multirow{2}{*}{QPP method}  & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20}  \\  
 \cmidrule(lr){2-4}  \cmidrule(lr){5-7} 
  & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$}  \\    
\midrule    
 Clarity & \textit{-0.078}  & \textit{-0.012} & \textit{-0.019} & \textit{-0.074}  & \textit{-0.048}  & \textit{-0.059} \\
 WIG & 0.313  & \textit{0.228} & \textit{0.286} & \textit{0.059}  & \textit{0.048} & \textit{0.053} \\  
 NQC & 0.350  & \textit{0.200} & \textit{0.251} & \textit{0.145} & \textit{0.112} & \textit{0.141}   \\  
 $\sigma_{max}$ & 0.384 & 0.287 & 0.348 & \textit{0.171}  & \textit{0.118} & \textit{0.157}   \\ 
 n($\sigma_{x\%}$) & \textit{0.200}  & \textit{0.176}  & \textit{0.217} & \textit{-0.008} & \textit{0.022} & \textit{0.024}   \\
 SMV  & 0.352 & 0.256  & 0.318 & \textit{0.182} & \textit{0.161} & \textit{0.205}  \\ 
\ac{QPP-PRP} &  &  &  &  &  &    \\
\midrule     
 NQA-QPP & \textit{-0.026}  & \textit{-0.009} & \textit{-0.005} & \textit{-0.059} & \textit{-0.080}  &  \textit{-0.095}    \\ 
 %NQA-QPP (train) & \textit{0.246} & \textit{0.204} & \textit{0.258} & \textit{0.036} & \textit{0.016} & \textit{0.025}    \\
  BERTQPP  & 0.330 & \textit{0.214} & \textit{0.261} & \textit{0.046} & \textit{-0.012} &   \textit{-0.031}   \\
% BERTQPP (train) & \textit{0.019}  & \textit{-0.033}  &  \textit{-0.026} & \textit{-0.008}  & \textit{-0.032}  & \textit{-0.045}   \\
 qppBERT-PL & \textit{0.092} & \textit{0.025}  & \textit{0.029} & \textit{-0.224} & \textit{-0.218}  & \textit{-0.230}  \\
 \ac{M-QPPF} &  &  &  &  &  &   \\
 \midrule 
\ourmodel & 0.567 & 0.440 & 0.476 & 0.293 & 0.257 & 0.296   \\
  \bottomrule
\end{tabular}
\end{table}





\subsection{Assess neural rankers}


\begin{table*}[]
\caption{
Correlation coefficients (Pearson's $\rho$, Kendall's $\tau$, and Spearman's $\rho$) between actual retrieval quality, in terms of nDCG@10, of BM25 and performance predicted by \ourmodel/baselines, on TREC-DL 19, 20, 21 and 22.
All coefficients are statistically significant (t-test, $p < 0.05$) except the ones in \emph{italics}.
The best value in each column is marked in \textbf{bold}.
}
\label{tab:RQ1}
\begin{tabular}{l rrr rrr rrr rrr}
\toprule
\multirow{2}{*}{QPP method}  & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20} & \multicolumn{3}{c}{TREC-DL 21} & \multicolumn{3}{c}{TREC-DL 22} \\
 \cmidrule(lr){2-4}  \cmidrule(lr){5-7}  \cmidrule(lr){8-10}   \cmidrule(lr){11-13}
  & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} \\    
\midrule 
 Clarity & \textit{0.091} & \textit{0.056}  & \textit{0.100}  & 0.358 & 0.250 & 0.345  & \textit{0.137} & \textit{0.078} & \textit{0.120}  & \textit{0.202}  & \textit{0.090} & \textit{0.133} \\
 WIG & 0.520 & 0.331 & 0.474 &  0.615  & 0.423 & 0.589 & 0.311 & 0.281  & 0.426  & 0.350  & 0.249  & 0.363 \\  
 NQC & 0.468 & 0.300  & 0.417  & 0.508 & 0.401 & 0.553  & \textit{0.134} & 0.221 & 0.338  & 0.360  & 0.156  & \textit{0.214} \\ 
 $\sigma_{max}$ & 0.478  & 0.327 & 0.448 & 0.529 & 0.440  & 0.610 & 0.298 & 0.258 & 0.372   & 0.142  & 0.196 & 0.274 \\  
 n($\sigma_{x\%}$)  & 0.532 & 0.311  & 0.480 & 0.622 & 0.443 & 0.620  & 0.328 & 0.234  &  0.362  & 0.336 & 0.228 & 0.329 \\
 SMV  & 0.376 & 0.271 & 0.360 & 0.463 & 0.383 & 0.537  & 0.327  & 0.236  & 0.343  & 0.338 & 0.155 & \textit{0.204} \\  
\ac{QPP-PRP} &  &  &  &  &  &  &  &  &   &  &  &   \\
\midrule 
 NQA-QPP &  \textit{0.210}  & \textit{0.147}  & \textit{0.201} &  \textit{0.244} & 0.210 & 0.319 & 0.286 & 0.201 & 0.322   & 0.312 & 0.194  & 0.293    \\ 
%NQA-QPP (train) & 0.331 & \textit{0.132} & \textit{0.202}  & 0.422 & 0.306 & 0.454 &  &  &   &  &  &    \\  
 BERTQPP  & 0.458 & \textit{0.207} & 0.308 & 0.426 & 0.300 & 0.421 &  0.351 & 0.223 & 0.323  & 0.369 & 0.229 & 0.331 \\
% BERTQPP (train) & 0.524 & 0.274  & 0.414  & 0.438 & 0.318 & 0.452  &  &  &   &  &  &    \\
 qppBERT-PL & \textit{0.171}  & \textit{0.175}  & \textit{0.227} & 0.410 & 0.279 & 0.380 & 0.277 & \textit{0.182}  & \textit{0.252}  & 0.300 & 0.242 & 0.325  \\
 \ac{M-QPPF} &  &  &  &  &  &  &  &  &   &  &  &  \\
 \midrule  
\ourmodel  & \textbf{0.715}  &  \textbf{0.477} &  \textbf{0.642} & \textbf{0.627} & \textbf{0.459}  & \textbf{0.601}    &  \textbf{0.550} & \textbf{0.440} & \textbf{0.610}  & \textbf{0.389} & \textbf{0.250} & \textbf{0.343} \\
  \bottomrule
\end{tabular}
\end{table*}



\begin{table}[]
\caption{
Correlation coefficients (Pearson's $\rho$, Kendall's $\tau$, and Spearman's $\rho$) between actual retrieval quality, in terms of nDCG@10, of ANCE and performance predicted by \ourmodel/baselines, on TREC-DL 19, 20.
All coefficients are statistically significant (t-test, $p < 0.05$) except the ones in \emph{italics}.
The best value in each column is marked in \textbf{bold}.
}   
\label{tab:RQ1}
\begin{tabular}{l rrr rrr}
\toprule
\multirow{2}{*}{QPP method}  & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20}  \\  
 \cmidrule(lr){2-4}  \cmidrule(lr){5-7} 
  & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$} & \multicolumn{1}{c}{P-$\rho$} & \multicolumn{1}{c}{K-$\tau$} & \multicolumn{1}{c}{S-$\rho$}  \\    
\midrule     
 Clarity & \textit{-0.088}  & \textit{-0.062} &  \textit{-0.065} & \textit{-0.091}  & \textit{-0.045} & \textit{-0.071} \\ 
 WIG    & 0.515 & 0.368  & 0.521 & \textit{0.218}  & \textit{0.150}  & \textit{0.227} \\
 NQC & 0.548 & 0.372 &  0.473 & 0.411 & 0.290 & 0.431   \\  
 $\sigma_{max}$ & 0.455 & 0.339 & 0.440 & 0.403 & 0.288  & 0.427 \\   
 n($\sigma_{x\%}$)& 0.388 & 0.315  & 0.467 & \textit{0.103}  & \textit{0.075}  & \textit{0.127} \\
 SMV & 0.496  & 0.359 & 0.474 & 0.380 & 0.283 & 0.422  \\ 
\ac{QPP-PRP} &  &  &  &  &  &    \\
\midrule  
 NQA-QPP  & \textit{0.089} & \textit{-0.038} & \textit{-0.036} & \textit{0.186} &  \textit{0.113} &  \textit{0.163}   \\
 %NQA-QPP (train) & \textit{0.073}  & \textit{0.055}  & \textit{0.060}  & \textit{0.154} & \textit{0.082} & \textit{0.120}    \\
 BERTQPP  & \textit{0.222} & \textit{0.117} & \textit{0.173} & \textit{0.137} & \textit{0.089} & \textit{0.130}    \\
% BERTQPP (train) & \textit{0.203}  & \textit{0.129}  & \textit{0.178}  & \textit{0.106} & \textit{0.078}  & \textit{0.117}    \\
 qppBERT-PL & \textit{0.116} & \textit{0.098} & \textit{0.118} & \textit{-0.119}  & \textit{-0.046}  & \textit{-0.056} \\ 
 \ac{M-QPPF} &  &  &  &  &  &   \\
 \midrule
\ourmodel & 0.719  & 0.492  & 0.655  & 0.447  & 0.321  & 0.459   \\
  \bottomrule
\end{tabular}
\end{table}



bm25
dl19 

n10-ndcg@10.ndcg@10: {'Pearson': 0.605, 'Kendall': 0.482, 'Spearman': 0.648,
n25-ndcg@10.ndcg@10: {'Pearson': 0.647, 'Kendall': 0.43, 'Spearman': 0.589
n50-ndcg@10.ndcg@10: {'Pearson': 0.677, 'Kendall': 0.453, 'Spearman': 0.617
n75-ndcg@10.ndcg@10: {'Pearson': 0.700, 'Kendall': 0.458, 'Spearman': 0.617
n100-ndcg@10.ndcg@10: {'Pearson': 0.712, 'Kendall': 0.472, 'Spearman': 0.632
n200-ndcg@10.ndcg@10: {'Pearson': 0.724, 'Kendall': 0.474, 'Spearman': 0.639
n300-ndcg@10.ndcg@10: {'Pearson': 0.726, 'Kendall': 0.476, 'Spearman': 0.641
n400-ndcg@10.ndcg@10: {'Pearson': 0.725, 'Kendall': 0.472, 'Spearman': 0.638
n500-ndcg@10.ndcg@10: {'Pearson': 0.722, 'Kendall': 0.470, 'Spearman': 0.637
n600-ndcg@10.ndcg@10: {'Pearson': 0.722, 'Kendall': 0.470, 'Spearman': 0.637
n700-ndcg@10.ndcg@10: {'Pearson': 0.722, 'Kendall': 0.470, 'Spearman': 0.637
n800-ndcg@10.ndcg@10: {'Pearson': 0.719, 'Kendall': 0.477, 'Spearman': 0.642
n900-ndcg@10.ndcg@10: {'Pearson': 0.715, 'Kendall': 0.477, 'Spearman': 0.642
n1000-ndcg@10.ndcg@10: {'Pearson': 0.715, 'Kendall': 0.477, 'Spearman': 0.642


bm25
dl20
n10-ndcg@10.ndcg@10: {'Pearson': 0.490, 'Kendall': 0.323, 'Spearman': 0.434
n25-ndcg@10.ndcg@10: {'Pearson': 0.547, 'Kendall': 0.394, 'Spearman': 0.521
n50-ndcg@10.ndcg@10: {'Pearson': 0.576, 'Kendall': 0.423, 'Spearman': 0.562
n75-ndcg@10.ndcg@10: {'Pearson': 0.587, 'Kendall': 0.439, 'Spearman': 0.575
n100-ndcg@10.ndcg@10: {'Pearson': 0.609, 'Kendall': 0.457, 'Spearman': 0.604
n200-ndcg@10.ndcg@10: {'Pearson': 0.638, 'Kendall': 0.469, 'Spearman': 0.625
n300-ndcg@10.ndcg@10: {'Pearson': 0.642, 'Kendall': 0.470, 'Spearman': 0.626
n400-ndcg@10.ndcg@10: {'Pearson': 0.643, 'Kendall': 0.473, 'Spearman': 0.628
n500-ndcg@10.ndcg@10: {'Pearson': 0.632, 'Kendall': 0.459, 'Spearman': 0.607
n600-ndcg@10.ndcg@10: {'Pearson': 0.627, 'Kendall': 0.455, 'Spearman': 0.599
n700-ndcg@10.ndcg@10: {'Pearson': 0.627, 'Kendall': 0.459, 'Spearman': 0.601
n800-ndcg@10.ndcg@10: {'Pearson': 0.627, 'Kendall': 0.459, 'Spearman': 0.601
n900-ndcg@10.ndcg@10: {'Pearson': 0.627, 'Kendall': 0.459, 'Spearman': 0.601
n1000-ndcg@10.ndcg@10: {'Pearson': 0.627, 'Kendall': 0.459, 'Spearman': 0.601

ance
dl19
n10-ndcg@10.ndcg@10: {'Pearson': 0.624, 'Kendall': 0.406, 'Spearman': 0.533
n25-ndcg@10.ndcg@10: {'Pearson': 0.700, 'Kendall': 0.492, 'Spearman': 0.638
n50-ndcg@10.ndcg@10: {'Pearson': 0.709, 'Kendall': 0.483, 'Spearman': 0.634
n75-ndcg@10.ndcg@10: {'Pearson': 0.701, 'Kendall': 0.480, 'Spearman': 0.632
n100-ndcg@10.ndcg@10: {'Pearson': 0.719, 'Kendall': 0.489, 'Spearman': 0.646
n200-ndcg@10.ndcg@10: {'Pearson': 0.712, 'Kendall': 0.483, 'Spearman': 0.642
n300-ndcg@10.ndcg@10: {'Pearson': 0.707, 'Kendall': 0.473, 'Spearman': 0.629
n400-ndcg@10.ndcg@10: {'Pearson': 0.719, 'Kendall': 0.492, 'Spearman': 0.657
n500-ndcg@10.ndcg@10: {'Pearson': 0.719, 'Kendall': 0.492, 'Spearman': 0.657
n600-ndcg@10.ndcg@10: {'Pearson': 0.720, 'Kendall': 0.494, 'Spearman': 0.657
n700-ndcg@10.ndcg@10: {'Pearson': 0.720, 'Kendall': 0.494, 'Spearman': 0.657
n800-ndcg@10.ndcg@10: {'Pearson': 0.720, 'Kendall': 0.494, 'Spearman': 0.657
n900-ndcg@10.ndcg@10: {'Pearson': 0.718, 'Kendall': 0.492, 'Spearman': 0.655,
n1000-ndcg@10.ndcg@10: {'Pearson': 0.719, 'Kendall': 0.492, 'Spearman': 0.655


ance
dl20
n10-ndcg@10.ndcg@10: {'Pearson': 0.306, 'Kendall': 0.238, 'Spearman': 0.343
n25-ndcg@10.ndcg@10: {'Pearson': 0.415, 'Kendall': 0.313, 'Spearman': 0.438
n50-ndcg@10.ndcg@10: {'Pearson': 0.432, 'Kendall': 0.321, 'Spearman': 0.445
n75-ndcg@10.ndcg@10: {'Pearson': 0.455, 'Kendall': 0.356, 'Spearman': 0.486
n100-ndcg@10.ndcg@10: {'Pearson': 0.456, 'Kendall': 0.355, 'Spearman': 0.481
n200-ndcg@10.ndcg@10: {'Pearson': 0.457, 'Kendall': 0.343, 'Spearman': 0.473
n300-ndcg@10.ndcg@10: {'Pearson': 0.455, 'Kendall': 0.335, 'Spearman': 0.468,
n400-ndcg@10.ndcg@10: {'Pearson': 0.457, 'Kendall': 0.333, 'Spearman': 0.468
n500-ndcg@10.ndcg@10: {'Pearson': 0.452, 'Kendall': 0.327, 'Spearman': 0.466
n600-ndcg@10.ndcg@10: {'Pearson': 0.452, 'Kendall': 0.328, 'Spearman': 0.466,
n700-ndcg@10.ndcg@10: {'Pearson': 0.452, 'Kendall': 0.328, 'Spearman': 0.466
n800-ndcg@10.ndcg@10: {'Pearson': 0.452, 'Kendall': 0.328, 'Spearman': 0.466
n900-ndcg@10.ndcg@10: {'Pearson': 0.452, 'Kendall': 0.328, 'Spearman': 0.466,
n1000-ndcg@10.ndcg@10: {'Pearson': 0.447, 'Kendall': 0.321, 'Spearman': 0.459


bm25
dl21
n10-ndcg@10.ndcg@10: {'Pearson': 0.497, 'Kendall': 0.384, 'Spearman': 0.532
n25-ndcg@10.ndcg@10: {'Pearson': 0.484, 'Kendall': 0.369, 'Spearman': 0.525
n50-ndcg@10.ndcg@10: {'Pearson': 0.525, 'Kendall': 0.402, 'Spearman': 0.572
n75-ndcg@10.ndcg@10: {'Pearson': 0.549, 'Kendall': 0.423, 'Spearman': 0.600
n100-ndcg@10.ndcg@10: {'Pearson': 0.549, 'Kendall': 0.428, 'Spearman': 0.606
n200-ndcg@10.ndcg@10: {'Pearson': 0.551, 'Kendall': 0.438, 'Spearman': 0.611
n300-ndcg@10.ndcg@10: {'Pearson': 0.548, 'Kendall': 0.437, 'Spearman': 0.607
n400-ndcg@10.ndcg@10: {'Pearson': 0.548, 'Kendall': 0.437, 'Spearman': 0.607
n500-ndcg@10.ndcg@10: {'Pearson': 0.549, 'Kendall': 0.437, 'Spearman': 0.606
n600-ndcg@10.ndcg@10: {'Pearson': 0.551, 'Kendall': 0.442, 'Spearman': 0.611
n700-ndcg@10.ndcg@10: {'Pearson': 0.549, 'Kendall': 0.437, 'Spearman': 0.607
n800-ndcg@10.ndcg@10: {'Pearson': 0.549, 'Kendall': 0.437, 'Spearman': 0.607
n900-ndcg@10.ndcg@10: {'Pearson': 0.549, 'Kendall': 0.437, 'Spearman': 0.607,
n1000-ndcg@10.ndcg@10: {'Pearson': 0.550, 'Kendall': 0.440, 'Spearman': 0.610


bm25
dl22
n10-ndcg@10.ndcg@10: {'Pearson': 0.316, 'Kendall': 0.245, 'Spearman': 0.335
n25-ndcg@10.ndcg@10: {'Pearson': 0.244, 'Kendall': 0.203, 'Spearman': 0.278
n50-ndcg@10.ndcg@10: {'Pearson': 0.267, 'Kendall': 0.226, 'Spearman': 0.304
n75-ndcg@10.ndcg@10: {'Pearson': 0.275, 'Kendall': 0.232, 'Spearman': 0.311
n100-ndcg@10.ndcg@10: {'Pearson': 0.284, 'Kendall': 0.233, 'Spearman': 0.31}
n200-ndcg@10.ndcg@10: {'Pearson': 0.290, 'Kendall': 0.234, 'Spearman': 0.306
n300-ndcg@10.ndcg@10: {'Pearson': 0.326, 'Kendall': 0.245, 'Spearman': 0.321
n400-ndcg@10.ndcg@10: {'Pearson': 0.327, 'Kendall': 0.245, 'Spearman': 0.323
n500-ndcg@10.ndcg@10: {'Pearson': 0.326, 'Kendall': 0.245, 'Spearman': 0.322
n600-ndcg@10.ndcg@10: {'Pearson': 0.325, 'Kendall': 0.245, 'Spearman': 0.321
n700-ndcg@10.ndcg@10: {'Pearson': 0.33, 'Kendall': 0.249, 'Spearman': 0.324
n800-ndcg@10.ndcg@10: {'Pearson': 0.332, 'Kendall': 0.246, 'Spearman': 0.322
n900-ndcg@10.ndcg@10: {'Pearson': 0.332, 'Kendall': 0.246, 'Spearman': 0.322,
n1000-ndcg@10.ndcg@10: {'Pearson': 0.332, 'Kendall': 0.246, 'Spearman': 0.322}

